The positivity-preserving high-order semi-Lagrangian spectral volume method for Vlasov-Poisson equations

In this paper, a novel high order semi-Lagrangian (SL) spectral volume (SV) method is proposed and studied for nonlinear Vlasov-Poisson (VP) simulations via operator splitting. The proposed algorithm combines both advantages of semi-Lagrangian and spectral volume approaches, exhibiting strong stability, robustness under large time steps, arbitrary high-order accuracy in space, local mass conservation, and positivity preservation. Numerical study of the SLSV method applied to the one-dimensional and two-dimensional transport equations, the Vlasov-Poisson system, the classical benchmark problems including Landau damping and two-stream instabilities is conducted, confirming the effectiveness, accuracy, and robustness of our algorithm in addressing complex nonlinear phenomena.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{multirow}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\newsiamremark{example}{Example}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{high order PP SLSV for VP}{X.Y. Zhang, X.F. Cai, and W.X. Cao}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{The positivity-preserving high-order semi-Lagrangian spectral volume method  for Vlasov-Poisson equations
\thanks{Submitted to the editors DATE.
\funding{This research is supported by National Natural Science Foundation of China under grants No. 12271049, 12201052, and
the Guangdong Provincial Key Laboratory of Inter-disciplinary Research and Application for Data Science of project code 2022B1212010006, BNBU Research Grant with No. of UICR0700035-22 at Beijing Normal-Hong Kong Baptist University,Zhuhai, PR China,
Guangdong basic and applied basic research foundation [2025A1515012182], National Key Laboratory for Computational Physics [6142A05230201].}}}

% Authors: full names plus addresses.
\author{Xinyue Zhang \thanks{Laboratory of Mathematics and Complex Systems, School of Mathematical Sciences, Beijing Normal University, Beijing, China  
  (\email{zhang\_xinyue@mail.bnu.edu.cn}).}
 \and Xiaofeng Cai \thanks{Research Center for Mathematics, Advanced Institute of Natural Sciences, Beijing Normal University, Zhuhai 519087, China; Guangdong Provincial/Zhuhai Key Laboratory of Interdisciplinary Research and Application for Data Science, Beijing Normal-Hong Kong Baptist University, Zhuhai 519087, China.
  (\email{xfcai@bnu.edu.cn}).}
 \and Waixiang Cao \thanks{Laboratory of Mathematics and Complex Systems, School of Mathematical Sciences, Beijing Normal University, Beijing, China  
 (\email{caowx@bnu.edu.cn}), corresponding author.}
}
\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

